Visualizing the Consequences of Climate Change Using Cycle-Consistent Adversarial Networks

We present a project that aims to generate images that depict accurate, vivid, and personalized outcomes of climate change using Cycle-Consistent Adversarial Networks (CycleGANs). By training our CycleGAN model on street-view images of houses before and after extreme weather events (e.g. floods, forest fires, etc.), we learn a mapping that can then be applied to images of locations that have not yet experienced these events. This visual transformation is paired with climate model predictions to assess likelihood and type of climate-related events in the long term (50 years) in order to bring the future closer in the viewers mind. The eventual goal of our project is to enable individuals to make more informed choices about their climate future by creating a more visceral understanding of the effects of climate change, while maintaining scientific credibility by drawing on climate model projections.

==> Ganify_CC_ICLR 2019-arxiv/Ideas&Links/ExtraLinksLitReview.tex <==
A key part of our project is bringing together the output of climate models with the generative capabilities of GANs to render images of the impact of climate change in a scientifically plausible manner. In order to do this, we based ourselves on existing climate maps~\citep{alfieri2015}, converting their output, which consists of statistical probabilities regarding extreme climate events, to binary values with regards to the likelihood of significant flooding in 2100 at a given GPS location defined by the viewer. We defined a threshold of X in order to be able to convert the discrete numbers outputted by the model into the binary flood model that we needed for our CycleGAN, and were therefore able to generate a binary flooding value at a given location with a granularity of Y meters. We then fed this value into the trained CycleGAN model, enabling it to generate a flooded house when the generated value was 1 and the Street View image of the address as-is when the value was 0.



%Localizing and detecting extreme events in large datasets is a major challenge in climate science research. Most algorithms for extreme event detection are based on human meteorologists defining subjective thresholds. Liu et al. \citeyearpar{liu2016} developed a CNN classification system coupled with a Bayesian based hyper-parameter optimization scheme by learning high-level representations to detect patterns such as tropical cyclones, atmospheric rivers and weather fronts, from labeled data. This work was extended further to localize climate patterns with semi-supervised bounding boxes with a multi-channel spatio-temporal CNN that was able to leverage temporal information and unlabeled data. The result improved the localization of extreme weather events and resulted in a new dataset for ML research whilst helping mitigate climate change impacts. Generating future frames, while using performance on a detection model to measure the quality of the generated frames could be an interesting future direction with GANs \citep{racah2017}. 

%Climate projections contain large uncertainties that stem from processes that need to be parameterized, such as clouds, convection, and ecosystems. With ML it is now possible to create climate model parameterization schemes (i.e. simplified physics models) and quantify uncertainties by matching low-order statistics that learn from climate models by integrating observations and local high-resolution simulations~\citep{schneider2017,}. In recent research at the nexus of ML and climate projection, Rasp et al.~\citeyearpar{rasp2018} demonstrated the use of deep learning in resolving sub-grid processes to create model clouds in place of existing heuristic-based parameterizations, whereas Scher et al.~\citeyearpar{scher2018} were able to approximate the dynamics of a simple climate model faithfully using a Convolutional Neural Network (CNN)~\citep{krizhevsky2012}, successfully predicting the time evolution of the model's state. Another application of ML in climate science is in tracking and predicting extreme events; for instance, Kim et al.~\citeyearpar{kim2018} recently used a convolutional Long-Short Term Memory Network (LSTM)~\citep{hochreiter1997} to model temporal dynamics and spatial distribution of hurricane trajectories from large climate data.
%O'Gorman and Dwyer~\citeyearpar{ogorman2018} used random forests to parameterize moist convection processes to emulate physical processes from expensive climate model outputs. 

%Moreover, interpretability and detecting new mechanisms are key to scientific discovery. 

%Predictive modeling of complex, nonlinear, and high-dimensional dynamical processes such as atmospheric convection are crucial for improving the reliability and accuracy of weather and climate models. Deep generative models have recently been successful in learning the underlying statistics of complex physical processes from large amounts of data. However, their success in predicting physical systems have been limited, primarily because they do not require physical consistency. By integrating physics constraints and desirable statistical properties into Generative Adversarial Networks (GANs)~\citep{goodfellow2014}, it might be possible to develop a new paradigm for modeling complex dynamical systems. Other ongoing research at the intersection of simulating physical processes and GANs have included the following investigations: high energy particle physics simulations of jet images~\citep{deoliveira2017}; predicting rapid flash fires for firefighters~\citep{yun2018}; state-parameter mapping for subsurface models; typhoon track prediction with satellite images~\citep{ruttgers2018}; flooded area segmentation from drone images~\citep{popescu2018,popescu2018b}. 

% For instance, Kim et al.~\citeyearpar{kim2018b} developed a novel generative model to synthesize fluid simulations from a set of reduced parameters. Their method was able to model a wide variety of fluid behaviors, thus enabling applications such as fast construction of simulations, interpolation of fluids with different parameters, time re-sampling, latent space simulations, and compression of fluid simulation data. 
% Also, in Xie et al.~\citeyearpar{xie2018}, four-dimensional physics fields were synthesized with neural networks. Based on a conditional GAN, their experiments inferred more realistic physical quantities, such as low-resolution velocities and vorticities. Finally, King et al.~\citeyearpar{king2018} trained deep learning neural network schemes on direct numerical simulations of turbulence. Their static deep learning scheme, implementing convolutional GANs and trained on spatial snapshots of turbulence, fails to reproduce intermittency of turbulent fluctuations at small scales and details of the turbulence geometry at large scales. However, their dynamic LAT-NET and compressed convolutional LSTM, trained on a temporal sequence of turbulence snapshots were able to correct for the issues with static neural networks. 

%Researchers have shown that behaviors and attitudes can be affected by interactions with decision calculators that visually depict the future consequences of actions taken today. For instance, we have found that young participants tend to save considerably more money when presented with a decision calculator that projects their income in retirement and is accompanied with an age-progressed photograph of themselves at retirement age \citep{hershfield2011}. Likewise, older employees intend to save more for retirement when their nest egg is made more vivid as a monthly amount to live on \citep{goldstein2016}. When people are given accurate depictions of how actions today affect outcomes tomorrow, they often change their behavior. In particular, they often behave more like people who have thought about the issues at length. This “decision aiding” approach maintains credibility by drawing on unbiased projections of the future, and leaving freedom of choice to the (now better informed) individual.

==> Ganify_CC_ICLR 2019-arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Ideas&Links/ExtraLinksLitReview.tex <==
A key part of our project is bringing together the output of climate models with the generative capabilities of GANs to render images of the impact of climate change in a scientifically plausible manner. In order to do this, we based ourselves on existing climate maps~\citep{alfieri2015}, converting their output, which consists of statistical probabilities regarding extreme climate events, to binary values with regards to the likelihood of significant flooding in 2100 at a given GPS location defined by the viewer. We defined a threshold of X in order to be able to convert the discrete numbers outputted by the model into the binary flood model that we needed for our CycleGAN, and were therefore able to generate a binary flooding value at a given location with a granularity of Y meters. We then fed this value into the trained CycleGAN model, enabling it to generate a flooded house when the generated value was 1 and the Street View image of the address as-is when the value was 0.



%Localizing and detecting extreme events in large datasets is a major challenge in climate science research. Most algorithms for extreme event detection are based on human meteorologists defining subjective thresholds. Liu et al. \citeyearpar{liu2016} developed a CNN classification system coupled with a Bayesian based hyper-parameter optimization scheme by learning high-level representations to detect patterns such as tropical cyclones, atmospheric rivers and weather fronts, from labeled data. This work was extended further to localize climate patterns with semi-supervised bounding boxes with a multi-channel spatio-temporal CNN that was able to leverage temporal information and unlabeled data. The result improved the localization of extreme weather events and resulted in a new dataset for ML research whilst helping mitigate climate change impacts. Generating future frames, while using performance on a detection model to measure the quality of the generated frames could be an interesting future direction with GANs \citep{racah2017}. 

%Climate projections contain large uncertainties that stem from processes that need to be parameterized, such as clouds, convection, and ecosystems. With ML it is now possible to create climate model parameterization schemes (i.e. simplified physics models) and quantify uncertainties by matching low-order statistics that learn from climate models by integrating observations and local high-resolution simulations~\citep{schneider2017,}. In recent research at the nexus of ML and climate projection, Rasp et al.~\citeyearpar{rasp2018} demonstrated the use of deep learning in resolving sub-grid processes to create model clouds in place of existing heuristic-based parameterizations, whereas Scher et al.~\citeyearpar{scher2018} were able to approximate the dynamics of a simple climate model faithfully using a Convolutional Neural Network (CNN)~\citep{krizhevsky2012}, successfully predicting the time evolution of the model's state. Another application of ML in climate science is in tracking and predicting extreme events; for instance, Kim et al.~\citeyearpar{kim2018} recently used a convolutional Long-Short Term Memory Network (LSTM)~\citep{hochreiter1997} to model temporal dynamics and spatial distribution of hurricane trajectories from large climate data.
%O'Gorman and Dwyer~\citeyearpar{ogorman2018} used random forests to parameterize moist convection processes to emulate physical processes from expensive climate model outputs. 

%Moreover, interpretability and detecting new mechanisms are key to scientific discovery. 

%Predictive modeling of complex, nonlinear, and high-dimensional dynamical processes such as atmospheric convection are crucial for improving the reliability and accuracy of weather and climate models. Deep generative models have recently been successful in learning the underlying statistics of complex physical processes from large amounts of data. However, their success in predicting physical systems have been limited, primarily because they do not require physical consistency. By integrating physics constraints and desirable statistical properties into Generative Adversarial Networks (GANs)~\citep{goodfellow2014}, it might be possible to develop a new paradigm for modeling complex dynamical systems. Other ongoing research at the intersection of simulating physical processes and GANs have included the following investigations: high energy particle physics simulations of jet images~\citep{deoliveira2017}; predicting rapid flash fires for firefighters~\citep{yun2018}; state-parameter mapping for subsurface models; typhoon track prediction with satellite images~\citep{ruttgers2018}; flooded area segmentation from drone images~\citep{popescu2018,popescu2018b}. 

% For instance, Kim et al.~\citeyearpar{kim2018b} developed a novel generative model to synthesize fluid simulations from a set of reduced parameters. Their method was able to model a wide variety of fluid behaviors, thus enabling applications such as fast construction of simulations, interpolation of fluids with different parameters, time re-sampling, latent space simulations, and compression of fluid simulation data. 
% Also, in Xie et al.~\citeyearpar{xie2018}, four-dimensional physics fields were synthesized with neural networks. Based on a conditional GAN, their experiments inferred more realistic physical quantities, such as low-resolution velocities and vorticities. Finally, King et al.~\citeyearpar{king2018} trained deep learning neural network schemes on direct numerical simulations of turbulence. Their static deep learning scheme, implementing convolutional GANs and trained on spatial snapshots of turbulence, fails to reproduce intermittency of turbulent fluctuations at small scales and details of the turbulence geometry at large scales. However, their dynamic LAT-NET and compressed convolutional LSTM, trained on a temporal sequence of turbulence snapshots were able to correct for the issues with static neural networks. 

%Researchers have shown that behaviors and attitudes can be affected by interactions with decision calculators that visually depict the future consequences of actions taken today. For instance, we have found that young participants tend to save considerably more money when presented with a decision calculator that projects their income in retirement and is accompanied with an age-progressed photograph of themselves at retirement age \citep{hershfield2011}. Likewise, older employees intend to save more for retirement when their nest egg is made more vivid as a monthly amount to live on \citep{goldstein2016}. When people are given accurate depictions of how actions today affect outcomes tomorrow, they often change their behavior. In particular, they often behave more like people who have thought about the issues at length. This “decision aiding” approach maintains credibility by drawing on unbiased projections of the future, and leaving freedom of choice to the (now better informed) individual.
